Is Hyper-Parameter Optimization Different for Software Analytics?

Yes. SE data can have "smoother" boundaries between classes (compared to traditional AI data sets). To be more precise, the magnitude of the second derivative of the loss function found in SE data is typically much smaller. A new hyper-parameter optimizer, called SMOOTHIE, can exploit this idiosyncrasy of SE data. We compare SMOOTHIE and a state-of-the-art AI hyper-parameter optimizer on three tasks: (a) GitHub issue lifetime prediction (b) detecting static code warnings false alarm; (c) defect prediction. For completeness, we also show experiments on some standard AI datasets. SMOOTHIE runs faster and predicts better on the SE data--but ties on non-SE data with the AI tool. Hence we conclude that SE data can be different to other kinds of data; and those differences mean that we should use different kinds of algorithms for our data. To support open science and other researchers working in this area, all our scripts and datasets are available on-line at https://github.com/yrahul3910/smoothness-hpo/.

==> conv.tex <==
\subsection{Convolutional classifiers}

This section focuses on convolutional neural networks that use max-pooling, ReLU activations in the intermediate layers, and a flattening layer after all convolutional layers that is fed to a one-layer feedforward network with a softmax activation. We also assume cross-entropy loss. These are standard settings that are used, and thus not strong assumptions.

\subsubsection{The architecture}

We assume that the network is comprised of Conv --$>$ ReLU --$>$ MaxPool blocks. The order of the ReLU and MaxPool, as we will later see, is not important. In this discussion, we will not include batch normalization or dropout.

Redefine $L$ to be the number of convolutional blocks, and at layer $l$, the input is convoluted with a kernel $k^{[l]}$, added to a bias vector $b^{[l]}$ (resulting in $z^{[l]}$), followed by a ReLU activation (resulting in $C^{[l]}$), and a max-pooling (resulting in $P^{[l]}$). After all convolutional layers, the output is flattened (resulting in $P^{[L]f}$), and passed to a feedforward network with weights $w$ and biases $b$, followed by a softmax layer.

In the forward propagation step, we perform the following (where $\lambda$ is the pooling parameter:
\begin{align}
    z^{[l]}_{muv} &= \sum\limits_n \sum\limits_n \sum\limits_q P^{[l-1]}_{n, p+u, q+v} k^{[l]}_{mnpq} + b^{[l]}_m \\
    C^{[l]}_{muv} &= \max (0, z^{[l]}_{muv}) \\
    P^{[l]}_{mxy} &= \max C^{[l]}_{muv} \\
    & u = \lambda x, \ldots, (\lambda + 1) x - 1 \\
    & v = \lambda y, \ldots, (\lambda + 1) y - 1
\end{align}

at the feedforward layer, we then do:
$$
S = \sum\limits_{j} w_{j} P^{[L]f} + b
$$

\begin{theorem}[Smoothness for convolutional classifiers]
    For a convolutional neural network whose intermediate activations are ReLU, and the output layer uses a softmax over the flattened activations of the penultimate layer, the {\smoothness} is given by
    $$
    \beta = \frac{\lVert P^{[L]} \rVert}{\lVert P^{[L]f} \rVert} \lVert w \rVert \lVert z^{[L-1]} \rVert
    $$
    for $w, P^{[L]}, P^{[L]f}$ as defined above.
\end{theorem}
\begin{proof}
    We have,
    \begin{align*}
        \frac{\partial \mathcal{L}}{\partial k^{[L]}_{mnpq}} &= \sum\limits_u \sum\limits_v \frac{\partial \mathcal{L}}{\partial z^{[L-1]}_{muv}} P^{[L-1]}_{n, p+u, q+v} \\
        %
        \frac{\partial \mathcal{L}}{\partial z^{[L]}_{muv}} &= \frac{\partial \mathcal{L}}{\partial C^{[L]}_{muv}} \frac{\partial C^{[L]}_{muv}}{\partial z^{[L]}_{muv}} \\
        %
        \frac{\partial C^{[L]}}{\partial z^{[L]}_{muv}} &\leq 1 \\
        %
        \frac{\partial \mathcal{L}}{\partial C^{[L]}_{muv}} &= \frac{\partial \mathcal{L}}{\partial P^{[L]}_{mxy}}
    \end{align*}
    where in the last equation, we have $x = \lfloor u/2 \rfloor, y = \lfloor v /2 \rfloor$, where $C^{[L]}_{muv} = \max C^{[L]}$. Next, we have

    \begin{align*}
        \frac{\partial \mathcal{L}}{\partial P^{[L]}} &= \text{reshape}\left( \frac{\partial \mathcal{L}}{\partial P^{[L]f}} \right) \\
        &= \text{reshape}\left( w^T \frac{\partial \mathcal{L}}{\partial S} \right)
    \end{align*}

    It can be shown that 
    $$
    \frac{\partial \mathcal{L}}{\partial S_i} = \begin{cases}
        O_{label} - 1 & \text{if } i = label \\
        O_i & \text{otherwise}
    \end{cases}
    $$
    so that $\lVert \frac{\partial \mathcal{L}}{\partial S} \rVert \leq c$.

    for some constant $c$ that we will ignore. We will now compute the Hessian with respect to $k$. We start with the first derivative.
    \begin{align*}
        \frac{\partial \mathcal{L}}{\partial k^{[L]}_{mnpq}} &\leq \frac{\partial \mathcal{L}}{\partial P^{[L]}} \frac{\partial P^{[L]}}{\partial k^{[L]}_{mnpq}} \\
        &\leq \sum\limits_u \sum\limits_v w^T P^{[L-1]}_{n, p+u, q+v} \\
        %
        \frac{\partial^2 \mathcal{L}}{\partial k^{[L]2}_{mnpq}} &\leq \sum\limits_u \sum\limits_v \left( \frac{\partial w^T}{\partial k^{[L]}_{mnpq}} P^{[L-1]}_{n, p+u, q+v} + w^T \frac{\partial P^{[L-1]}_{n, p+u, q+v}}{\partial k^{[L]}_{mnpq}} \right)
    \end{align*}
    The latter term is zero since there is no forward dependence in the system. For brevity, we will, from now on, work in vectorized notation.
    \begin{align}
        \left\lVert \nabla^2_k \mathcal{L} \right\rVert &\leq \left\lVert \frac{\partial w^T}{\partial k^{[L]}} \right\rVert \left\lVert P^{[L-1]} \right\rVert \nonumber \\
        &\leq \left\lVert \frac{\partial w^T}{\partial k^{[L]}} \right\rVert \left\lVert C^{[L-1]} \right\rVert \nonumber \\
        &\leq \left\lVert \frac{\partial w^T}{\partial k^{[L]}} \right\rVert \left\lVert z^{[L-1]} \right\rVert \label{eq:conv:hess}
    \end{align}
    We have,
    \begin{align*}
        \frac{\partial w}{\partial k^{[L]}} &= \frac{\partial w}{\partial S} \frac{\partial S}{\partial z^{[L]}} \frac{\partial z^{[L]}}{\partial k^{[L]}} \\
        &= \frac{1}{\frac{\partial S}{\partial w}} \frac{\partial S}{\partial z^{[L]}} P^{[L]}
    \end{align*}
    Note that we ignore the transpose since $\lVert w^T \rVert = \lVert w \rVert$. Applying the norm on both sides,
    \begin{align*}
        \frac{\partial w}{\partial k^{[L]}} &= \frac{1}{\left \lVert P^{[L]f} \right\rVert} \left\lVert \frac{\partial S}{\partial z^{[L]}} \right\rVert \left\lVert P^{[L]} \right\rVert \\
        &= \frac{\left\lVert P^{[L]} \right\rVert}{\left\lVert P^{[L]f} \right\rVert} \left\lVert \frac{\partial S}{\partial P^{[L]}} \frac{\partial P^{[L]}}{\partial C^{[L]}} \frac{\partial C^{[L]}}{\partial z^{[L]}} \right\rVert
    \end{align*}
    The last two terms are bounded by 1, and $\left\lVert \frac{\partial S}{\partial P^{[L]}} \right\rVert = \lVert w \rVert$. Combining with \eqref{eq:conv:hess} yields our final result.
\end{proof}

==> old.tex <==
Off-the-shelf learners contain hyper-parameters that generally do not suit the current data set well. Hyper-parameter optimization (HPO) is the process of automatically tuning those parameters. In practice, such optimizations can lead to dramatic improvements in learner performance.

HPO can be an excessively CPU intensive process that might need to be repeated when learners or data change.
In this paper we ask what have we learned from our
prior HPO work that might simplify that optimization process.
Our starting point for that is Figure \ref{fig:smooth} which shows experiments in improving quality predictors for software engineering~\cite{yedida2023find}.  In that figure, $x,y$ are two random projections and $Z$ shows the loss function for examples
taken from that domain. The right-hand side of that figure is ``smoother'' and was found after applying a set of data pre-processors that tried to fix problem areas in the data For example, examples too close to the hyperspace boundary between classes can be misclassified due to noise. Hence in the local region at those points we synthesized artificial examples of the same class as the threatened examples
(for more these operators, see \S\ref{sec:hyperparams}). In that case study, we found dramatic improvements in predictive performance in the smoothed data.


Off-the-shelf learners contain hyper-parameters that generally do not suit the current data set well. Hyper-parameter optimization (HPO) is the process of automatically tuning those parameters. In practice, such optimizations can lead to dramatic improvements in learner performance.

HPO can be an excessively CPU intensive process that might need to be repeated when learners or data change.
In this paper we ask what have we learned from our
prior HPO work that might simplify that optimization process.
Our starting point for that is Figure \ref{fig:smooth} which shows experiments in improving quality predictors for software engineering~\cite{XXXtse}.  In that figure, $x,y$ are two random projections and $Z$ shows the loss function for examples
taken from that domain. The right-hand side of that figure is ``smoother'' and was found after applying a set of data pre-processors that tried to fix problem areas in the data For example, examples too close to the hyperspace boundary between classes can be misclassified due to noise. Hence in the local region at those points we synthesized artificial examples of the same class as the threatened examples
(for more these operators, see \S\ref{XXX}). In that case study, we found dramatic improvements in predictive performance in the smoothed data.

While an encouraging result, that prior work was somewhat ad-hoc. From a library of data pre-processors we used ``engineering judgement''
(i.e. we guessed) what operators to apply. In this paper we ask if the selection of pre-processor can be automated. 
Specifically, instead of running a  deep learner for
(say) $N \geq 100 $ epochs, we rank candidate pre-processor by the  $\beta$-smoothness 
(defined in \S\ref{XXX}) seen in their loss function 
generated after just $N=1$ epoch.  The five
top-ranked items are then executed and we return the best.   It turns this procedure is no slower than  state of the art hyper-parameter optimizers~\cite{lee2020continual}  yet achieves
dramatically better results. For example,
as shown by the experiments of this paper,
we have results where the    accuracy increased from 43\% to 71.9\% 
(median values seen in 20 repeated trials). 

We argue that $\beta$-smoothness  is a general
heuristic for improving hyper-parameter optimization.
To demonstrate this, we apply the method to a range of 
learners (deep learning, logistic regression, and Naive Bayes).
For example:
\bi 
\item 
Gradient descent in logistic regression (LR) converges after $N={\approx}30$  epochs. We find after  $N=1$ epochs we can use smoothness to select five best    data pre-processing operators for LR. From that reduced
set, we can tune   logistic regression to perform better than  a state-of-the-art neural approach~\cite{lee2020continual}
(especially in $k>2$ class problems).
\item For Naive Bayes applied to
  software defect prediction, models built from
  data generated via our 
$\beta$-smoothness method, work as or better than state-of-art neural methods. 
\ei 
The rest of this paper is structured as follows.xxx 
we use 2020 NeurIPS Black-Box Optimization Challenge \cite{cowen2022hebo, turner2021bayesian}
mentone the optimizer you comapre against.
